The Neural Network First-Level Hardware Track Trigger of the Belle II Experiment

We describe the principles and performance of the first-level ("L1") hardware track trigger of Belle II, based on neural networks. The networks use as input the results from the standard Belle II trigger, which provides "2D" track candidates in the plane transverse to the electron-positron beams. The networks then provide estimates for the origin of the 2D track candidates in direction of the colliding beams ("$z$-vertex"), as well as their polar emission angles $\theta$. Given the $z$-vertices of the "neural" tracks allows identifying events coming from the collision region ($z \approx 0$), and suppressing the overwhelming background from outside by a suitable cut $d$. Requiring $|z| < d$ for at least one neural track in an event with two or more 2D candidates will set an L1 trigger. The networks also enable a minimum bias trigger, requiring a single 2D track candidate validated by a neural track with a momentum larger than 0.7 GeV in addition to the $|z|$ condition. The momentum of the neural track is derived with the help of the polar angle $\theta$.

==> monitoring.tex <==

A comprehensive package of simulation and hardware monitoring software for the neural operation, including live control plots for the ongoing runs, has been developed. The package is running at the pure software High Level Trigger (HLT) level and includes the reconstructed tracks, so that a direct comparison between the reconstructed quantities and their neural estimates can be made. The package is also used for offline quality control where it is running on a subset of events written to tape in special format (``CDST'') by the HLT trigger (see next chapter).

At present, the set of online plots collects the 2D-input and the set of TSs (axial and stereo) to the neural hardware and produces plots for the neural output ($z$ and $\cos(\theta)$). A few examples of the online output are given here for runs at the beginning (high background) and at the end (low background) of the 2021c data taking (see fig.~\ref{fig:online}).


\begin{figure}[!ht]
\begin{center}
\begin{minipage}[hbt]{0.48\linewidth}
\centering
\includegraphics[width=1.0\textwidth]{./images/DQMExp16R633Z0.pdf}
\includegraphics[width=1.0\textwidth]{./images/DQMExp16R633Cost.pdf}
%\includegraphics[width=1.0\textwidth]{./images/DQMExp16R633Clks.pdf}
\end{minipage}
\hfill
\begin{minipage}[hbt]{0.48\linewidth}
\centering
\includegraphics[width=1.0\textwidth]{./images/DQMExp22R406Z0.pdf}
\includegraphics[width=1.0\textwidth]{./images/DQMExp22R406Cost.pdf}
%\includegraphics[width=1.0\textwidth]{./images/DQMExp22R406Clks.pdf}
\end{minipage}
\caption{
  Online distributions for the neural tracks found at level 1. The left column is from run 633 in Exp. 16 (March 2, 2021), and the right column is from run 406 in exp. 22, Dec. 12, 2021. 
  In Exp. 16, the neural trigger was not yet active (see the high background from tracks at large $z$). The neural trigger became active by the end of March, 2021. The right column shows the distributions close to the end of the 2021c running. The dashed lines are the reference distributions taken from an earlier run in Exp. 16.    
}
\label{fig:online} 
\end{center}
\end{figure}

As is evident from the left column of fig.~\ref{fig:online} the strong peak at $z = 60$ cm can be rejected by a cut on the $z$-output of the networks. Correspondingly, the enhancement in $\cos(\theta) < 0$ (backward direction) supports the fact that the neural tracks from $z = 60$ cm (tip of the final focusing superconducting quadrupole QCSR) are "real" in the sense that they are scattered into the backward hemisphere (second row of histograms). Compare the column on the right side: Here the neural $z$-trigger was active and the majority of the tracks from the QCSR tip are rejected. Accordingly, the $\cos(\theta)$ distribution looks more "physical", i.e. with emission angles dominantly into the forward direction, as expected from the boost in the laboratory system. The small rate of tracks at large $z$ demonstrates the ability of the neural trigger to reject this background efficiently. 

The third row in fig.~\ref{fig:online} shows the clock counter number, when the $z$-trigger information is actually arriving at the General Decision Logic (GDL). There are two interesting features: first, there are two peaks in the clock distribution, where the second one - according to the trigger experts - is caused by a re-sending of the 2D tracks to the neural system. This second peak will be worked on and should finally disappear. The other effect is the difference between the peak position in Exp.16 in comparison to Exp. 18: The shift indicates a fluctuation in the latency of the system: One clock cycle equals 32 ns; here, the shift is small, but was observed to reach values of up to about 160 ns. According to the 2D/GDL trigger experts this should not be a problem, but will also be subject of further investigations. 

